LinguAlchemy: Fusing Typological and Geographical Elements for Unseen Language Generalization

Pretrained language models (PLMs) have become remarkably adept at task and language generalization. Nonetheless, they often fail when faced with unseen languages. In this work, we present LinguAlchemy, a regularization method that incorporates various linguistic information covering typological, geographical, and phylogenetic features to align PLMs representation to the corresponding linguistic information on each language. Our LinguAlchemy significantly improves the performance of mBERT and XLM-R on low-resource languages in multiple downstream tasks such as intent classification, news classification, and semantic relatedness compared to fully finetuned models and displaying a high degree of unseen language generalization. We further introduce AlchemyScale and AlchemyTune, extension of LinguAlchemy which adjusts the linguistic regularization weights automatically, alleviating the need for hyperparameter search.

==> maintable.tex <==

\begin{table}[t]
\resizebox{.48\textwidth}{!}{
\begin{tabular}{@{}l|rrr|lll}
\toprule
                 & \multicolumn{3}{c}{\textbf{mBERT}}                                                               & \multicolumn{2}{c}{\textbf{XLM-R}} \\
\textbf{Language} &
  \textbf{AF} &
  \textbf{Full FT} &
  \textbf{Ours} &
  \textbf{Full FT} &
  \textbf{Ours} \\
\midrule
am-ET*            & \cellcolor[HTML]{E06666}4.61\%  & \cellcolor[HTML]{E06868}5.45\%  & \cellcolor[HTML]{8CACDF}58.07\% & \cellcolor[HTML]{AEBFDB}78.55\% & \cellcolor[HTML]{BDC8D9}77.00\% \\
cy-GB            & \cellcolor[HTML]{E0ABA8}25.05\% & \cellcolor[HTML]{E0A7A4}23.81\% & \cellcolor[HTML]{E0BCB8}30.01\% & \cellcolor[HTML]{E09693}64.39\% & \cellcolor[HTML]{E0B9B4}68.96\% \\
af-ZA            & \cellcolor[HTML]{8EADDF}57.67\% & \cellcolor[HTML]{A4B9DC}52.72\% & \cellcolor[HTML]{AFBFDB}50.16\% & \cellcolor[HTML]{85A8E0}82.72\% & \cellcolor[HTML]{CACFD7}75.73\% \\
km-KH*            & \cellcolor[HTML]{E07170}7.83\%  & \cellcolor[HTML]{E07272}8.34\%  & \cellcolor[HTML]{85A7E0}59.85\% & \cellcolor[HTML]{739EE2}84.57\% & \cellcolor[HTML]{ADBEDB}78.70\% \\
sw-KE            & \cellcolor[HTML]{E0A19E}22.16\% & \cellcolor[HTML]{E09997}19.77\% & \cellcolor[HTML]{9AB4DD}54.93\% & \cellcolor[HTML]{E06666}58.07\% & \cellcolor[HTML]{D2D3D6}74.90\% \\
mn-MN*            & \cellcolor[HTML]{E0B4B0}27.57\% & \cellcolor[HTML]{E0B3AF}27.17\% & \cellcolor[HTML]{8FAEDF}57.38\% & \cellcolor[HTML]{568DE6}87.53\% & \cellcolor[HTML]{C4CCD8}76.27\% \\
tl-PH            & \cellcolor[HTML]{DAD8D5}40.25\% & \cellcolor[HTML]{E0D6D0}37.46\% & \cellcolor[HTML]{6897E4}66.47\% & \cellcolor[HTML]{6696E4}85.91\% & \cellcolor[HTML]{9CB5DD}80.42\% \\
kn-IN            & \cellcolor[HTML]{D7D6D6}40.99\% & \cellcolor[HTML]{E0CBC6}34.23\% & \cellcolor[HTML]{6294E5}67.84\% & \cellcolor[HTML]{9BB4DD}80.46\% & \cellcolor[HTML]{94B0DE}81.19\% \\
te-IN            & \cellcolor[HTML]{E0CBC6}34.40\% & \cellcolor[HTML]{E0CEC9}35.27\% & \cellcolor[HTML]{508AE7}71.88\% & \cellcolor[HTML]{739EE2}84.57\% & \cellcolor[HTML]{87A9E0}82.59\% \\
sq-AL            & \cellcolor[HTML]{B2C1DA}49.53\% & \cellcolor[HTML]{C7CDD8}44.75\% & \cellcolor[HTML]{558DE6}70.66\% & \cellcolor[HTML]{E0B1AD}67.92\% & \cellcolor[HTML]{8BABDF}82.17\% \\
ur-PK            & \cellcolor[HTML]{BCC7D9}47.11\% & \cellcolor[HTML]{CFD2D7}42.80\% & \cellcolor[HTML]{5B90E5}69.43\% & \cellcolor[HTML]{DFDAD5}73.60\% & \cellcolor[HTML]{8EADDF}81.81\% \\
az-AZ            & \cellcolor[HTML]{739EE2}63.82\% & \cellcolor[HTML]{7DA3E1}61.57\% & \cellcolor[HTML]{5C90E5}69.18\% & \cellcolor[HTML]{9EB6DD}80.16\% & \cellcolor[HTML]{8CACDF}82.03\% \\
ml-IN            & \cellcolor[HTML]{E0D0CB}35.84\% & \cellcolor[HTML]{E0B4B0}27.71\% & \cellcolor[HTML]{6294E5}67.83\% & \cellcolor[HTML]{ABBDDB}78.92\% & \cellcolor[HTML]{8EADDF}81.80\% \\
ms-MY            & \cellcolor[HTML]{6A99E3}65.80\% & \cellcolor[HTML]{6897E4}66.48\% & \cellcolor[HTML]{6194E5}67.85\% & \cellcolor[HTML]{83A6E0}82.99\% & \cellcolor[HTML]{8EADDF}81.80\% \\
ca-ES            & \cellcolor[HTML]{4B87E7}73.07\% & \cellcolor[HTML]{4A86E8}73.10\% & \cellcolor[HTML]{5F92E5}68.37\% & \cellcolor[HTML]{588EE6}87.36\% & \cellcolor[HTML]{8CACDF}82.04\% \\
sl-SL            & \cellcolor[HTML]{B3C2DA}49.29\% & \cellcolor[HTML]{BCC7D9}47.18\% & \cellcolor[HTML]{5F92E5}68.52\% & \cellcolor[HTML]{6394E4}86.28\% & \cellcolor[HTML]{8BABDF}82.15\% \\
sv-SE            & \cellcolor[HTML]{729DE3}64.09\% & \cellcolor[HTML]{84A7E0}60.05\% & \cellcolor[HTML]{5F92E5}68.36\% & \cellcolor[HTML]{6B99E3}85.37\% & \cellcolor[HTML]{8AABDF}82.20\% \\
ta-IN            & \cellcolor[HTML]{D4D5D6}41.66\% & \cellcolor[HTML]{E0CDC8}34.87\% & \cellcolor[HTML]{5E92E5}68.63\% & \cellcolor[HTML]{759EE2}84.43\% & \cellcolor[HTML]{89AAE0}82.38\% \\
nl-NL            & \cellcolor[HTML]{588EE6}69.97\% & \cellcolor[HTML]{558DE6}70.65\% & \cellcolor[HTML]{5E92E5}68.62\% & \cellcolor[HTML]{8DACDF}81.98\% & \cellcolor[HTML]{89AAE0}82.34\% \\
it-IT            & \cellcolor[HTML]{508AE7}71.86\% & \cellcolor[HTML]{558CE6}70.78\% & \cellcolor[HTML]{6093E5}68.14\% & \cellcolor[HTML]{B0C0DB}78.31\% & \cellcolor[HTML]{8BABDF}82.14\% \\
he-IL            & \cellcolor[HTML]{AABDDB}51.24\% & \cellcolor[HTML]{B8C4DA}48.18\% & \cellcolor[HTML]{6193E5}68.07\% & \cellcolor[HTML]{4A86E8}88.74\% & \cellcolor[HTML]{8AAADF}82.25\% \\
pl-PL            & \cellcolor[HTML]{7AA1E1}62.27\% & \cellcolor[HTML]{84A7E0}59.99\% & \cellcolor[HTML]{6596E4}67.05\% & \cellcolor[HTML]{E07E7D}61.30\% & \cellcolor[HTML]{90AEDF}81.60\% \\
da-DK            & \cellcolor[HTML]{538BE6}71.25\% & \cellcolor[HTML]{518AE7}71.72\% & \cellcolor[HTML]{6897E4}66.39\% & \cellcolor[HTML]{C3CBD8}76.46\% & \cellcolor[HTML]{92AFDE}81.43\% \\
nb-NO            & \cellcolor[HTML]{5E91E5}68.76\% & \cellcolor[HTML]{5F92E5}68.53\% & \cellcolor[HTML]{6B99E3}65.71\% & \cellcolor[HTML]{B2C1DA}78.18\% & \cellcolor[HTML]{93B0DE}81.33\% \\
ro-RO            & \cellcolor[HTML]{8AAADF}58.68\% & \cellcolor[HTML]{9DB5DD}54.20\% & \cellcolor[HTML]{6E9BE3}64.93\% & \cellcolor[HTML]{84A7E0}82.82\% & \cellcolor[HTML]{93AFDE}81.34\% \\
th-TH            & \cellcolor[HTML]{E0BEB9}30.43\% & \cellcolor[HTML]{E0A8A5}24.21\% & \cellcolor[HTML]{719CE3}64.37\% & \cellcolor[HTML]{E0DAD4}73.30\% & \cellcolor[HTML]{96B1DE}81.05\% \\
fa-IR            & \cellcolor[HTML]{87A9E0}59.35\% & \cellcolor[HTML]{91AFDF}56.89\% & \cellcolor[HTML]{719CE3}64.38\% & \cellcolor[HTML]{BBC6D9}77.20\% & \cellcolor[HTML]{96B1DE}81.04\% \\
\textbf{Average} & 47.95\%                         & 45.48\%                         & \textbf{64.19\%}                & 78.97\%                & \textbf{80.32\%} \\
\bottomrule
\end{tabular}
}
\caption{Performance of \methodname~in MASSIVE dataset for unseen languages. These models have not seen these languages during fine-tuning. For languages in *, mBERT model also never seen the languages during pre-training.}
\label{tab:maintable}
\end{table}
